Till the Layers Collapse: Compressing a Deep Neural Network through the Lenses of Batch Normalization Layers

Today, deep neural networks are widely used since they can handle a variety of complex tasks. Their generality makes them very powerful tools in modern technology. However, deep neural networks are often overparameterized. The usage of these large models consumes a lot of computation resources. In this paper, we introduce a method called \textbf{T}ill the \textbf{L}ayers \textbf{C}ollapse (TLC), which compresses deep neural networks through the lenses of batch normalization layers. By reducing the depth of these networks, our method decreases deep neural networks' computational requirements and overall latency. We validate our method on popular models such as Swin-T, MobileNet-V2, and RoBERTa, across both image classification and natural language processing (NLP) tasks.

==> sections/main_table.tex <==
\begin{table*}[!ht]
    \centering
    \begin{tabular}{c c c c c c c c c c c}
    \toprule
    \multirow{2}{*}{\bf Dataset}  & \multirow{2}{*}{\bf Approach} &\multicolumn{3}{c}{\bf ResNet-18}&\multicolumn{3}{c}{\bf MobileNet-V2}&\multicolumn{3}{c}{\bf Swin-T}\\
     &  & $\widehat{\mathcal{H}}_{\text{min}}$ & top-1 & Rem.& $\widehat{\mathcal{H}}_{\text{min}}$ & top-1 & Rem.& $\widehat{\mathcal{H}}_{\text{min}}$ & top-1 & Rem.\\
    \midrule
    \multirow{11}{*}{CIFAR-10} & Dense model & 0.647 & 91.66 & 0/17 & 0.386 & 93.68 & 0/35 & 0.028 & 91.54 & 0/12 \\
    %\cmidrule{2-11}
    &Smallest weights & 0.582 & 10.00 &  1/17 & 0 & 10.00 & 1/35 & 0.031 & 89.22 & 2/12\\
    &Smallest gradients & 0.314 & 9.29 & 1/17 & 0 & 10.00 & 1/35 & 0.03 & 89.21 & 2/12\\
    &Group lasso & 0.130 & 92.11 & 1/17 & 0.001 & 83.00 & 4/35 & 0.028 & 91.68 & 0/12\\
    &IMP \small{(low prune)} & 0.585 & 92.29 & 0/17 & 0.186 & 94.07 & 0/35 & 0.001 & 91.73 & 0/12\\
    &IMP \small{(mid prune)}& 0.192 & 92.27 & 0/17 & 0.063 & 93.32 & 0/35 & 0.001 & 91.46 & 0/12 \\
    &IMP \small{(high prune)}& 0.055 & 91.66 & 0/17 & 0.046 & 93.50 & 0/35 & 0.286 & 90.53 & 0/12\\
    %\cmidrule{2-11}
    &EGP & - & 92.18 & 3/17 & - & 92.22 & 6/35 & - & 92.01 & 1/12\\
    &Layer folding & - & 90.65 & 1/17 & - & 87.84 & 6/35 & - & 85.73 & 2/12\\
    &\it NEPENTHE  &\it 0.121 &\it 92.55 &\it 3/17 &\it 0.001 &\it 93.26 &\it 7/35 &\it 0.362 &\it 92.29 &\it 2/12\\
    \midrule
    %%%%%%%%%%%%%%%%% TINY IMAGENET %%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%% TINY IMAGENET %%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%% TINY IMAGENET %%%%%%%%%%%%%%%
    \multirow{11}{*}{Tiny-ImageNet} & Dense model & 0.471 & 41.44 & 0/17 & 0.076 & 45.86 & 0/35 & 0.067 & 75.60 & 0/12 \\
    %\cmidrule{2-11}
    &Smallest weights & 0 & 0.5 & 1/17 & 0 & 0.5 & 1/35 & 0.07 & 75.12 & 1/12\\
    &Smallest gradients & 0 & 0.5 & 1/17 & 0.099 & 46.62 & 1/35 & 0.07 & 74.54 & 1/12\\
    &Group lasso & 0.418 & 41.92 & 0/17 & 0.001 & 47.1 & 0/35 & 0.124 & 71.3 & 0/12\\
    &IMP \small{(low prune)} & 0.470 & 42.24 & 0/17 & 0.036 & 45.84 & 0/35 & 0.069 & 75.86 & 0/12\\
    &IMP \small{(mid prune)}  & 0.485 & 41.18 & 0/17 & 0.161 & 46.80 & 0/35 & 0.089 & 75.32 & 0/12 \\
    &IMP \small{(high prune)} & 0.464 & 39.14 & 0/17 & 0.013 & 45.24 & 0/35 & 0.104 & 67.56 & 0/12\\
    %\cmidrule{2-11}
    &EGP & - & 39.50 & 4/17 & - & 47.52 & 6/35 & - & 71.48 & 1/12\\
    &Layer folding & - & 37.86 & 4/17 & - & 25.88 & 12/35 & - & 50.54 & 1/12\\
    &\it NEPENTHE  &\it 0.129 &\it 39.56 &\it 5/17 &\it 0.002 &\it 47.92 &\it 12/35 &\it 0.126 &\it 72.58 &\it 1/12\\
    \midrule
    %%%%%%%%%%%%%%%%% PACS %%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%% PACS %%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%% PACS %%%%%%%%%%%%%%%
    \multirow{11}{*}{PACS} & Dense model & 0.332 & 94.70 & 0/17 & 0.207 & 93.20 & 0/35 & 0.057 & 97.10 & 0/12 \\
    %\cmidrule{2-11}
    &Smallest weights & 0.122 & 16.20 & 1/17 & 0 & 18.5 & 1/35 & 0.078 & 96.1 & 2/12\\
    &Smallest gradients & 0.115 & 16.20 & 1/17 & 0.063 & 16.2 & 1/35 & 0.069 & 95.7 & 2/12\\
    &Group lasso & 0.831 & 81.2 & 0/17 & 0.176 & 95.10 & 0/35 & 0.063 & 96.3 & 0/12\\
    &IMP \small{(low prune)} & 0.331 & 95.40 & 0/17 & 0.218 & 95.70 & 0/35 & 0.060 & 96.60 & 0/12\\
    &IMP \small{(mid prune)}  & 0.319 & 95.10 & 0/17 & 0.222 & 95.70 & 0/35 & 0.095 & 96.60 & 0/12 \\
    & IMP \small{(high prune)}& 0.280 & 90.80 & 0/17 & 0.170 & 95.40 & 0/35 & 0.101 & 93.90 & 0/12\\
    %\cmidrule{2-11}
    &EGP & - & 84.30 & 2/17 & - & 17.7 & 3/35 & - & 93.5 & 1/12\\
    &Layer folding & - & 82.90 & 3/17 & - & 79.70 & 1/35 & - & 87.70 & 2/12\\
    &\it NEPENTHE  &\it 0.030 &\it 90.10 &\it 3/17 &\it 0.080 &\it 92.20 &\it 1/35 &\it 0.335 &\it 95.10 &\it 2/12\\
    \midrule
    %%%%%%%%%%%%%%%%% VLCS %%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%% VLCS %%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%% VLCS %%%%%%%%%%%%%%%
    \multirow{11}{*}{VLCS} & Dense model & 0.382 & 80.89 & 0/17 & 0.258 & 81.83 & 0/35 & 0.070 & 86.58 & 0/12 \\
    %\cmidrule{2-11}
    &Smallest weights & 0.122 & 46.13 & 1/17 & 0 & 6.43 & 1/35 & 0.063 & 84.62 & 1/12\\
    &Smallest gradients & 0.122 & 46.13 & 1/17 & 0.176 & 46.13 & 1/35 & 0.064 & 84.15 & 1/12\\
    &Group lasso & 0.831 & 67.85 & 0/17 & 0.176 & 78.84 & 0/35 & 0.063 & 84.81 & 0/12\\
    &IMP \small{(low prune)} & 0.387 & 82.79 & 0/17 & 0.269 & 80.80 & 0/35 & 0.078 & 84.72 & 0/12\\
    &IMP \small{(mid prune)}  & 0.391 & 80.15 & 0/17 & 0.258 & 79.59 & 0/35 & 0.122 & 84.06 & 0/12 \\   
    &IMP \small{(high prune)} & 0.357 & 74.09 & 0/17 & 0.273 & 80.43 & 0/35 & 0.139 & 80.06 & 0/12\\
    %\cmidrule{2-11}
    &EGP & - & 74.28 & 2/12 & - & 45.85 & 2/35 & - & 82.95 & 1/12\\
    &Layer folding & - & 64.87 & 1/17 & - & 68.87 & 2/35 & - & 70.92 & 1/12\\
    &\it NEPENTHE  &\it 0.224 &\it 78.38 &\it 2/17 &\it 0.001 &\it 80.06 &\it 2/35 &\it 0.411 &\it 85.27 &\it 1/12\\
    \midrule
    %%%%%%%%%%%%%%%%% SVIRO %%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%% SVIRO %%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%% SVIRO %%%%%%%%%%%%%%%
    \multirow{11}{*}{SVIRO} & Dense model & 0.336 & 99.93 & 0/17 & 0.187 & 99.95 & 0/35 & 0.060 & 99.95 & 0/12 \\
    %\cmidrule{2-11}
    &Smallest weights & 0.122 & 35.55 & 1/12 & 0.014 & 35.55 & 1/35 & 0.039 & 99.70 & 4/12\\
    &Smallest gradients & 0.122 & 35.55 & 1/12 & 0.014 & 35.55 & 1/35 & 0.0154 & 99.55 & 4/12\\
    &Group lasso & 0.803 & 99.77 & 0/12 & 0.795 & 99.93 & 0/35 & 0.014 & 99.79 & 0/35\\
    &IMP \small{(low prune)} & 0.327 & 99.98 & 0/17 & 0.165 & 99.98 & 0/35 & 0.046 & 99.84 & 0/12\\
    &IMP \small{(mid prune)}  & 0.335 & 99.95 & 0/17 & 0.169 & 99.96 & 0/35 & 0.027 & 99.68 & 0/12 \\
    &IMP \small{(high prune)} & 0.308 & 99.95 & 0/17 & 0.146 & 99.95 & 0/35 & 0.260 & 99.75 & 0/12\\
    %\cmidrule{2-11}
    &EGP & - & 99.88 & 5/17 & - & 35.05 & 2/35 & - & 99.64 & 5/35\\
    &Layer folding & - & 99.46 & 8/17 & - & 99.83 & 2/35 & - & 99.66 & 5/12\\
    &\it NEPENTHE  &\it 0.001 &\it 99.61 &\it 8/17 &\it 0.020 &\it 99.98 &\it 2/35 &\it 0.162 &\it 99.75 &\it 5/12\\
    \bottomrule
    \end{tabular}
    \caption{Test performance (top-1), lowest non-zero layers' entropy ($\widehat{\mathcal{H}}_{\text{min}}$) and the number of removed layers (Rem.) for all the considered Image classification setups. The results achieved by our method are in italic.}
    \label{tab:results_image_class}
\end{table*}




\begin{table*}[!ht]
    \centering
    \begin{tabular}{c c c c c c c c c c c}
    \toprule
    \multirow{2}{*}{\bf Dataset}  & \multirow{2}{*}{\bf Approach} &\multicolumn{3}{c}{\bf BERT}&\multicolumn{3}{c}{\bf RoBERTa}\\
     &  & $\widehat{\mathcal{H}}_{\text{min}}$ & top-1 & Rem.& $\widehat{\mathcal{H}}_{\text{min}}$ & top-1 & Rem.\\
    \midrule
    %%%%%%%%%%%%%%%%% QNLI %%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%% QNLI %%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%% QNLI %%%%%%%%%%%%%%%    
    \multirow{5}{*}{QNLI} & Dense model & 0.173 & 90.48 & 0/12 & 0.190 & 92.18 & 0/12  \\
    %\cmidrule{2-11}
    &IMP \small{(low prune)} & 0.215 & 89.80 & 0/12 & 0.216 & 91.56 & 0/12   \\
    &IMP \small{(mid prune)} & 0.265 & 89.15 & 0/12 & 0.239 & 90.19 & 0/12 \\
    &IMP \small{(high prune)} & 0.307 & 85.87 & 0/12 & 0.263 & 89.04 & 0/12  \\
    %\cmidrule{2-11}
    &\it NEPENTHE  &\it 0.251 &\it 88.69 &\it 4/12 &\it 0.001 &\it 87.41 &\it 2/12 \\
    \midrule

    %%%%%%%%%%%%%%%%% RTE %%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%% RTE %%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%% RTE %%%%%%%%%%%%%%%
    \multirow{5}{*}{RTE} & Dense model & 0.211 & 61.01 & 0/12 & 0.236 & 66.787 & 0/12  \\
    %\cmidrule{2-11}
    &IMP \small{(low prune)} & 0.258 & 59.21 & 0/12 & 0.249 & 66.06 & 0/12  \\
    &IMP \small{(mid prune)} & 0.287 & 58.48 & 0/12 & 0.285 & 64.98 & 0/12 \\
    &IMP \small{(high prune)} & 0.335 & 57.76 & 0/12 & 0.314 & 62.82 & 0/12   \\
    %\cmidrule{2-11}
    &\it NEPENTHE  &\it 0.001 &\it 58.12 &\it 4/12 &\it 0.001 &\it 66.06 &\it 1/12 \\
    \midrule
    %%%%%%%%%%%%%%%%% SST-2 %%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%% SST-2 %%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%% SST-2 %%%%%%%%%%%%%%%
    \multirow{5}{*}{SST-2} & Dense model & 0.114 & 92.202 & 0/12 & 0.131 & 92.66 & 0/12  \\
    %\cmidrule{2-11}
    &IMP \small{(low prune)} & 0.187 & 87.96 & 0/12 & 0.177 & 91.17 & 0/12  \\
    &IMP \small{(mid prune)} & 0.329 & 84.75 & 0/12 & 0.178 & 88.99 & 0/12 \\
    &IMP \small{(high prune)} & 0.301 & 83.94 & 0/12 & 0.125 & 87.16 & 0/12  \\
    %\cmidrule{2-11}
    &\it NEPENTHE  &\it 0.001 &\it 82.11 &\it 5/12 &\it 0.001 &\it 87.5 &\it 5/12 \\
    \bottomrule
    \end{tabular}
    \caption{Test performance (top-1), lowest non-zero layers' entropy ($\widehat{\mathcal{H}}_{\text{min}}$) and the number of removed layers (Rem.) for all the considered NLP setups. The results achieved by our method are in italic.}
    \label{tab:results_nlps}
\end{table*}
